Modeling accretion shocks at the disk-envelope interface -- Sulfur chemistry

As material from an infalling protostellar envelope hits the forming disk, an accretion shock may develop which could (partially) alter the envelope material entering the disk. Observations with the Atacama Large Millimeter/submillimeter Array (ALMA) indicate that emission originating from warm SO and SO$_2$ might be good tracers of such accretion shocks. The goal of this work is to test under what shock conditions the abundances of gas-phase SO and SO$_2$ increase in an accretion shock at the disk-envelope interface. Detailed shock models including gas dynamics are computed using the Paris-Durham shock code for non-magnetized J-type accretion shocks in typical inner envelope conditions. The effect of pre-shock density, shock velocity, and strength of the ultraviolet (UV) radiation field on the abundance of warm SO and SO$_2$ is explored. Warm gas-phase chemistry is efficient in forming SO under most J-type shock conditions considered. In lower-velocity (~3 km/s) shocks, the abundance of SO is increased through subsequent reactions starting from thermally desorbed CH$_4$ toward H$_2$CO and finally SO. In higher velocity (>4 km/s) shocks, both SO and SO$_2$ are formed through reactions of OH and atomic S. The strength of the UV radiation field is crucial for SO and in particular SO$_2$ formation through the photodissociation of H$_2$O. Thermal desorption of SO and SO$_2$ ice is only relevant in high-velocity (>5 km/s) shocks at high densities ($>10^7$ cm$^{-3}$). Warm emission from SO and SO$_2$ is a possible tracer of accretion shocks at the disk-envelope interface as long as a local UV field is present. Additional observations with ALMA at high-angular resolution could provide further constraints. Moreover, the James Webb Space Telescope will give access to other possible slow, dense shock tracers such as H$_2$, H$_2$O, and [S I] 25$\mu$m.

==> OLD_input_abundances.tex <==
\longtab[1]{
\begin{longtable}{ll|ll|ll|ll}
\caption{Dark cloud input abundances} \\
\hline \hline
Species & Abundance & Species & Abundance & Species & Abundance & Species & Abundance \\
\hline
\endfirsthead
\hline\hline
Species & Abundance & Species & Abundance & Species & Abundance & Species & Abundance \\
\hline
\endhead
\hline
\endfoot
$\rm H$          & $5.0 \times 10^{-5}$   & $\rm CS$         & $3.0 \times 10^{-9}$   & $\rm Fe**$       & $3.2 \times 10^{-5}$   & $\rm NH_4^+$     & $1.0 \times 10^{-20}$ \\
$\rm H_2$        & $5.0 \times 10^{-1}$   & $\rm SO$         & $1.0 \times 10^{-9}$   & $\rm C**$        & $1.6 \times 10^{-4}$   & $\rm CN^+$       & $1.0 \times 10^{-20}$ \\
$\rm He$         & $1.0 \times 10^{-1}$   & $\rm SO_2$       & $1.0 \times 10^{-9}$   & $\rm H^+$        & $1.0 \times 10^{-20}$  & $\rm C_2N^+$     & $1.0 \times 10^{-20}$ \\
$\rm C$          & $1.0 \times 10^{-8}$   & $\rm OCS$        & $2.0 \times 10^{-9}$   & $\rm H_2^+$      & $1.0 \times 10^{-20}$  & $\rm HCN^+$      & $1.0 \times 10^{-20}$ \\
$\rm CH$         & $1.0 \times 10^{-20}$  & $\rm Si$         & $1.0 \times 10^{-10}$  & $\rm H_3^+$      & $1.0 \times 10^{-20}$  & $\rm H_2CN^+$    & $1.0 \times 10^{-20}$ \\
$\rm CH_2$       & $1.0 \times 10^{-20}$  & $\rm SiH$        & $1.0 \times 10^{-20}$  & $\rm He^+$       & $1.0 \times 10^{-20}$  & $\rm H_2NC^+$    & $1.0 \times 10^{-20}$ \\
$\rm CH_3$       & $1.0 \times 10^{-20}$  & $\rm SiH_2$      & $1.0 \times 10^{-20}$  & $\rm C^+$        & $1.0 \times 10^{-20}$  & $\rm N_2^+$      & $1.0 \times 10^{-20}$ \\
$\rm CH_4$       & $1.0 \times 10^{-20}$  & $\rm SiH_3$      & $1.0 \times 10^{-20}$  & $\rm CH^+$       & $1.0 \times 10^{-20}$  & $\rm N_2H^+$     & $1.0 \times 10^{-20}$ \\
$\rm O$          & $1.0 \times 10^{-6}$   & $\rm SiH_4$      & $1.0 \times 10^{-20}$  & $\rm CH_2^+$     & $1.0 \times 10^{-20}$  & $\rm NO^+$       & $1.0 \times 10^{-20}$ \\
$\rm O_2$        & $1.0 \times 10^{-20}$  & $\rm SiO$        & $1.0 \times 10^{-20}$  & $\rm CH_3^+$     & $1.0 \times 10^{-20}$  & $\rm HNO^+$      & $1.0 \times 10^{-20}$ \\
$\rm OH$         & $1.0 \times 10^{-20}$  & $\rm SiO_2$      & $1.0 \times 10^{-20}$  & $\rm CH_4^+$     & $1.0 \times 10^{-20}$  & $\rm S^+$        & $1.0 \times 10^{-20}$ \\
$\rm H_2O$       & $1.0 \times 10^{-20}$  & $\rm Mg$         & $1.0 \times 10^{-20}$  & $\rm CH_5^+$     & $1.0 \times 10^{-20}$  & $\rm SH^+$       & $1.0 \times 10^{-20}$ \\
$\rm CO$         & $8.5 \times 10^{-5}$   & $\rm Fe$         & $1.5 \times 10^{-8}$   & $\rm O^+$        & $1.0 \times 10^{-20}$  & $\rm H_2S^+$     & $1.0 \times 10^{-20}$ \\
$\rm HCO$        & $1.0 \times 10^{-20}$  & $\rm PAH$        & $1.0 \times 10^{-8}$   & $\rm O_2^+$      & $1.0 \times 10^{-20}$  & $\rm H_3S^+$     & $1.0 \times 10^{-20}$ \\
$\rm CO_2$       & $1.0 \times 10^{-20}$  & $\rm G$          & $4.6 \times 10^{-11}$  & $\rm OH^+$       & $1.0 \times 10^{-20}$  & $\rm CS^+$       & $1.0 \times 10^{-20}$ \\
$\rm C_2$        & $1.0 \times 10^{-20}$  & $\rm H_2O*$      & $1.0 \times 10^{-4}$   & $\rm H_2O^+$     & $1.0 \times 10^{-20}$  & $\rm HCS^+$      & $1.0 \times 10^{-20}$ \\
$\rm C_2H$       & $2.0 \times 10^{-9}$   & $\rm O_2*$       & $1.0 \times 10^{-8}$   & $\rm H_3O^+$     & $1.0 \times 10^{-20}$  & $\rm SO^+$       & $1.0 \times 10^{-20}$ \\
$\rm C_2H_2$     & $1.0 \times 10^{-20}$  & $\rm CO*$        & $8.3 \times 10^{-6}$   & $\rm CO^+$       & $1.0 \times 10^{-20}$  & $\rm HSO^+$      & $1.0 \times 10^{-20}$ \\
$\rm C_3$        & $1.0 \times 10^{-20}$  & $\rm CO_2*$      & $1.3 \times 10^{-5}$   & $\rm HCO^+$      & $1.5 \times 10^{-9}$   & $\rm HSO_2^+$    & $1.0 \times 10^{-20}$ \\
$\rm C_3H$       & $1.0 \times 10^{-20}$  & $\rm CH_4*$      & $1.5 \times 10^{-6}$   & $\rm H_2CO^+$    & $1.0 \times 10^{-20}$  & $\rm HOCS^+$     & $1.0 \times 10^{-20}$ \\
$\rm C_3H_2$     & $2.0 \times 10^{-10}$  & $\rm N_2*$       & $3.9 \times 10^{-6}$   & $\rm H_3CO^+$    & $1.0 \times 10^{-20}$  & $\rm Si^+$       & $1.0 \times 10^{-20}$ \\
$\rm CH_3OH$     & $1.5 \times 10^{-9}$   & $\rm NH_3*$      & $1.0 \times 10^{-6}$   & $\rm CH_3OH^+$   & $1.0 \times 10^{-20}$  & $\rm SiH^+$      & $1.0 \times 10^{-20}$ \\
$\rm H_2CO$      & $1.0 \times 10^{-20}$  & $\rm CH_3OH*$    & $1.9 \times 10^{-5}$   & $\rm CH_5O^+$    & $1.0 \times 10^{-20}$  & $\rm SiH_2^+$    & $1.0 \times 10^{-20}$ \\
$\rm HCO_2H$     & $1.0 \times 10^{-20}$  & $\rm H_2CO*$     & $6.2 \times 10^{-6}$   & $\rm HCO_2^+$    & $1.0 \times 10^{-20}$  & $\rm SiH_3^+$    & $1.0 \times 10^{-20}$ \\
$\rm N$          & $1.0 \times 10^{-6}$   & $\rm HCO_2H*$    & $7.2 \times 10^{-6}$   & $\rm C_2^+$      & $1.0 \times 10^{-20}$  & $\rm SiH_4^+$    & $1.0 \times 10^{-20}$ \\
$\rm NH$         & $1.0 \times 10^{-20}$  & $\rm OCS*$       & $2.1 \times 10^{-7}$   & $\rm C_2H^+$     & $1.0 \times 10^{-20}$  & $\rm SiH_5^+$    & $1.0 \times 10^{-20}$ \\
$\rm NH_2$       & $1.0 \times 10^{-20}$  & $\rm H_2S*$      & $1.8 \times 10^{-5}$   & $\rm C_2H_2^+$   & $1.0 \times 10^{-20}$  & $\rm SiO^+$      & $1.0 \times 10^{-20}$ \\
$\rm NH_3$       & $1.0 \times 10^{-20}$  & $\rm SO*$        & $1.0 \times 10^{-7}$   & $\rm C_2H_3^+$   & $1.0 \times 10^{-20}$  & $\rm SiOH^+$     & $1.0 \times 10^{-20}$ \\
$\rm CN$         & $1.5 \times 10^{-9}$   & $\rm SO_2*$      & $1.0 \times 10^{-7}$   & $\rm C_3^+$      & $1.0 \times 10^{-20}$  & $\rm Fe^+$       & $1.0 \times 10^{-20}$ \\
$\rm HCN$        & $3.0 \times 10^{-9}$   & $\rm SiH_4*$     & $1.0 \times 10^{-20}$  & $\rm C_3H^+$     & $1.0 \times 10^{-20}$  & $\rm PAH^+$      & $1.0 \times 10^{-20}$ \\
$\rm HNC$        & $1.0 \times 10^{-9}$   & $\rm SiO*$       & $1.0 \times 10^{-20}$  & $\rm C_3H_2^+$   & $1.0 \times 10^{-20}$  & $\rm G^+$        & $1.0 \times 10^{-20}$ \\
$\rm N_2$        & $3.5 \times 10^{-5}$   & $\rm SiO_2*$     & $1.0 \times 10^{-20}$  & $\rm C_3H_3^+$   & $1.0 \times 10^{-20}$  & $\rm PAH^-$      & $1.0 \times 10^{-20}$ \\
$\rm NO$         & $1.0 \times 10^{-20}$  & $\rm Fe*$        & $1.0 \times 10^{-20}$  & $\rm N^+$        & $1.0 \times 10^{-20}$  & $\rm G^-$        & $1.0 \times 10^{-20}$ \\
$\rm S$          & $6.0 \times 10^{-7}$   & $\rm O**$        & $1.4 \times 10^{-4}$   & $\rm NH^+$       & $1.0 \times 10^{-20}$  & $\rm H^-$        & $1.0 \times 10^{-20}$ \\
$\rm SH$         & $1.0 \times 10^{-20}$  & $\rm Si**$       & $3.4 \times 10^{-5}$   & $\rm NH_2^+$     & $1.5 \times 10^{-10}$  & $\rm Mg^+$       & $1.0 \times 10^{-20}$ \\
$\rm H_2S$       & $1.0 \times 10^{-9}$   & $\rm Mg**$       & $3.7 \times 10^{-5}$   & $\rm NH_3^+$     & $1.0 \times 10^{-20}$ \\
$\rm CS$         & $3.0 \times 10^{-9}$   & $\rm Fe**$       & $3.2 \times 10^{-5}$   & $\rm NH_4^+$     & $1.0 \times 10^{-20}$ \\
\hline
\end{longtable}
\tablefoot{Abundances are with respect to \nH. Species in ice mantles on dust grains are indicated with a *. Species in composing the cores of dust grains are indicated with **.}
\label{tab:input_abundances}
}
